Neural Microfacet Fields for Inverse Rendering

We present Neural Microfacet Fields, a method for recovering materials, geometry, and environment illumination from images of a scene. Our method uses a microfacet reflectance model within a volumetric setting by treating each sample along the ray as a (potentially non-opaque) surface. Using surface-based Monte Carlo rendering in a volumetric setting enables our method to perform inverse rendering efficiently by combining decades of research in surface-based light transport with recent advances in volume rendering for view synthesis. Our approach outperforms prior work in inverse rendering, capturing high fidelity geometry and high frequency illumination details; its novel view synthesis results are on par with state-of-the-art methods that do not recover illumination or materials.

==> eqns.tex <==
\boldsymbol{\omega}_k\sim D(\alpha, \boldsymbol{n}) \\
L_s = \frac1N\sum_{k=1}^N L(\boldsymbol{p}, \boldsymbol{\omega}_k) h(\boldsymbol{p}, \boldsymbol{\omega}_k, \boldsymbol{\omega}_o) \\
\lambda(\boldsymbol{p}) \\
L_o \\
\boldsymbol{E}(\boldsymbol{n})=\frac1\pi\int_{\Omega(\boldsymbol{n})}L(\boldsymbol{\omega})(\boldsymbol{\omega}\cdot\boldsymbol{n})d\boldsymbol{\omega} \\

==> tables/ablations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{l|rrrr}
             & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{$\text{MAE}^\circ \downarrow$} \\ \hline
%PhySG$^1$                     & 26.21                               & .921                                & .121                                   & 8.46                                              \\
%NVDiffRec$^1$                 & 29.90                               & .945                                & .114                                   & 6.08                                              \\
%NVDiffRecMC$^1$               & 28.20                               & .902                                & .175                                   & 4.93                                              \\
Ours, no integral image & 32.11                               & 0.950                                & 0.077                                   & 2.51                      \\
Ours, single bounce       & 32.86                               & 0.957                                & 0.067                                   & 2.60                                              \\

Ours, no $L_d$            & 31.69                               & 0.888                                & 0.242                                   & 4.37                                              \\
Ours, no smoothing        & 31.20                               & 0.942                                & 0.092                                   & 5.01                                              \\
Ours                & \textbf{33.24}                               & \textbf{0.960}                                & \textbf{0.062}                                   & \textbf{2.41}
\end{tabular}

==> tables/blender_metrics.tex <==
% \begin{tabular}{l|rrr}
% Blender     & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} \\
% \hline
% PhySG (requires masks)      & 18.538                              & 0.847                               & 0.182                                  \\
% NVDiffRec (requires masks)  & 28.787                              & 0.939                               & 0.068                                  \\
% NVDiffRecMC (requires masks) & 25.812                              & 0.904                               & 0.111                                  \\
% Ref-NeRF    & 33.994                              & 0.966                               & 0.038                                  \\
% Ours        & 30.702                              & 0.943                               & 0.047                                 
% \end{tabular}

% \begin{tabular}{l|cccc}
% Blender     & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{$\text{MAE}^\circ \downarrow$} \\ \hline
% PhySG$^1$       & 18.538                              & 0.847                               & 0.182                                  & 29.170                                            \\
% NVDiffRec$^1$   & 28.787                              & 0.939                               & 0.068                                  & 7.795                                             \\
% NVDiffRecMC$^1$ & 25.812                              & 0.904                               & 0.111                                  & 7.094                                             \\
% Ref-NeRF    & \textbf{33.994}                              & \textbf{0.966}                               & 0.038                                  & 23.220                    \\
% Ours        & 30.702                              & 0.943                               & \textbf{0.047}                                  & \textbf{5.274}                                            
% \end{tabular}

\begin{tabular}{l|rrrr}
    & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{$\text{MAE}^\circ \downarrow$} \\ \hline
PhySG$^1$       & 18.54                              & 0.847                               & 0.182                                  & 29.17                                            \\
NVDiffRec$^1$   & 28.79                              & 0.939                               & 0.068                                  & 7.80                                             \\
NVDiffRecMC$^1$ & 25.81                              & 0.904                               & 0.111                                  & 7.09                                             \\
Ref-NeRF$^2$    & \textbf{33.99}                              & \textbf{0.966}                               & \textbf{0.038}                                  & 23.22                    \\
Ours        & 30.70                              & 0.943                               & 0.047                                  & \textbf{5.27}                                            
\end{tabular}

==> tables/relighting_full.tex <==
\begin{tabular}{l|rrrrrrr}
PSNR $\uparrow$    & \multicolumn{1}{l}{toaster}   & \multicolumn{1}{l}{coffee}    & \multicolumn{1}{l}{helmet}    & \multicolumn{1}{l}{ball}      & \multicolumn{1}{l}{teapot}    & \multicolumn{1}{l}{car}       & \multicolumn{1}{l}{mean}       \\ \hline
NVDiffRec$^1$      & \cellcolor[HTML]{FFFFB4}12.56 & 20.30                         & \cellcolor[HTML]{FFFFB4}17.73 & 13.21                         & \cellcolor[HTML]{FFFFB4}33.00 & 19.84                         & 19.44                          \\
NVDiffRecMC$^1$    & \cellcolor[HTML]{FFD9B3}14.55 & \cellcolor[HTML]{FFD9B3}23.39 & \cellcolor[HTML]{FFD9B3}20.44 & \cellcolor[HTML]{FFFFB4}13.23 & 32.51                         & \cellcolor[HTML]{FFFFB4}20.09 & \cellcolor[HTML]{FFFFB4}20.70  \\
Control            & 12.45                         & \cellcolor[HTML]{FFB3B3}24.89 & 17.13                         & \cellcolor[HTML]{FFD9B3}13.90 & \cellcolor[HTML]{FFB3B3}36.54 & \cellcolor[HTML]{FFD9B3}20.89 & \cellcolor[HTML]{FFD9B3}20.966 \\
Ours               & \cellcolor[HTML]{FFB3B3}19.78 & \cellcolor[HTML]{FFFFB4}23.28 & \cellcolor[HTML]{FFB3B3}25.12 & \cellcolor[HTML]{FFB3B3}25.27 & \cellcolor[HTML]{FFD9B3}34.23 & \cellcolor[HTML]{FFB3B3}22.96 & \cellcolor[HTML]{FFB3B3}25.11  \\ \hline
LPIPS $\downarrow$ & \multicolumn{1}{l}{toaster}   & \multicolumn{1}{l}{coffee}    & \multicolumn{1}{l}{helmet}    & \multicolumn{1}{l}{ball}      & \multicolumn{1}{l}{teapot}    & \multicolumn{1}{l}{car}       & \multicolumn{1}{l}{mean}       \\ \hline
NVDiffRec$^1$      & .378                          & .208                          & .229                          & .467                          & .027                          & .113                          & .237                           \\
NVDiffRecMC$^1$    & \cellcolor[HTML]{FFFFB4}.290  & \cellcolor[HTML]{FFFFB4}.177  & \cellcolor[HTML]{FFFFB4}.217  & \cellcolor[HTML]{FFFFB4}.423  & \cellcolor[HTML]{FFFFB4}.024  & \cellcolor[HTML]{FFFFB4}.105  & \cellcolor[HTML]{FFFFB4}.206   \\
Control            & \cellcolor[HTML]{FFD9B3}.263  & \cellcolor[HTML]{FFB3B3}.143  & \cellcolor[HTML]{FFD9B3}.186  & \cellcolor[HTML]{FFD9B3}.316  & \cellcolor[HTML]{FFD9B3}.021  & \cellcolor[HTML]{FFD9B3}.075  & \cellcolor[HTML]{FFD9B3}.167   \\
Ours               & \cellcolor[HTML]{FFB3B3}.163  & \cellcolor[HTML]{FFD9B3}.145  & \cellcolor[HTML]{FFB3B3}.103  & \cellcolor[HTML]{FFB3B3}.171  & \cellcolor[HTML]{FFB3B3}.018  & \cellcolor[HTML]{FFB3B3}.057  & \cellcolor[HTML]{FFB3B3}.110   \\ \hline
SSIM $\uparrow$    & \multicolumn{1}{l}{toaster}   & \multicolumn{1}{l}{coffee}    & \multicolumn{1}{l}{helmet}    & \multicolumn{1}{l}{ball}      & \multicolumn{1}{l}{teapot}    & \multicolumn{1}{l}{car}       & \multicolumn{1}{l}{mean}       \\ \hline
NVDiffRec$^1$      & .624                          & .870                          & .824                          & .626                          & .985                          & .853                          & .797                           \\
NVDiffRecMC$^1$    & \cellcolor[HTML]{FFD9B3}.741  & \cellcolor[HTML]{FFFFB4}.913  & \cellcolor[HTML]{FFFFB4}.861  & \cellcolor[HTML]{FFFFB4}.761  & \cellcolor[HTML]{FFFFB4}.986  & \cellcolor[HTML]{FFFFB4}.869  & \cellcolor[HTML]{FFFFB4}.855   \\
Control            & \cellcolor[HTML]{FFFFB4}.735  & \cellcolor[HTML]{FFD9B3}.922  & \cellcolor[HTML]{FFD9B3}.874  & \cellcolor[HTML]{FFD9B3}.830  & \cellcolor[HTML]{FFB3B3}.990  & \cellcolor[HTML]{FFD9B3}.893  & \cellcolor[HTML]{FFD9B3}.874   \\
Ours               & \cellcolor[HTML]{FFB3B3}.860  & \cellcolor[HTML]{FFB3B3}.925  & \cellcolor[HTML]{FFB3B3}.937  & \cellcolor[HTML]{FFB3B3}.916  & \cellcolor[HTML]{FFD9B3}.987  & \cellcolor[HTML]{FFB3B3}.923  & \cellcolor[HTML]{FFB3B3}.925  
\end{tabular}

==> tables/shiny_blender_metrics.tex <==
% \begin{tabular}{@{}l|rrrr}
% Shiny Blender & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{$\text{MAE}^\circ \downarrow$} \\ \hline
% PhySG$^1$       & 26.213                              & 0.921                               & 0.121                                  & 8.460                                             \\
% NVDiffRec$^1$     & 29.896                              & 0.945                               & 0.114                                  & 6.080                                             \\
% NVDiffRecMC$^1$  & 28.199                              & 0.902                               & 0.175                                  & 4.930                                             \\
% Ref-NeRF      & 35.962                              & 0.967                               & 0.059                                  & 18.380                                            \\
% Ours          & 33.477                              & 0.961                               & 0.059                                  & 2.395      
% \end{tabular}


\begin{tabular}{@{}l|rrrr}
 & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{$\text{MAE}^\circ \downarrow$} \\ \toprule
PhySG$^1$       & 26.21                              & 0.921                               & 0.121                                  & 8.46                                             \\
NVDiffRec$^1$     & 29.90                              & 0.945                               & 0.114                                  & 6.08                                             \\
NVDiffRecMC$^1$  & 28.20                              & 0.902                               & 0.175                                  & 4.93                                             \\
Ref-NeRF$^2$      & \textbf{35.96}                              & \textbf{0.967}                               & \textbf{0.059}                                  & 18.38                                            \\
Ours          & 33.48                              & 0.961                               & \textbf{0.059}                                  & \textbf{2.40}      
\end{tabular}
